The FHD/$\boldsymbol{\varepsilon}$ppsilon Epoch of Reionization Power Spectrum Pipeline

Epoch of Reionization data analysis requires unprecedented levels of accuracy in radio interferometer pipelines. We have developed an imaging power spectrum analysis to meet these requirements and generate robust 21 cm EoR measurements. In this work, we build a signal path framework to mathematically describe each step in the analysis, from data reduction in the FHD package to power spectrum generation in the $\varepsilon$ppsilon package. In particular, we focus on the distinguishing characteristics of FHD/$\varepsilon$ppsilon: highly accurate spectral calibration, extensive data verification products, and end-to-end error propagation. We present our key data analysis products in detail to facilitate understanding of the prominent systematics in image-based power spectrum analyses. As a verification to our analysis, we also highlight a full-pipeline analysis simulation to demonstrate signal preservation and lack of signal loss. This careful treatment ensures that the FHD/$\varepsilon$ppsilon power spectrum pipeline can reduce radio interferometric data to produce credible 21 cm EoR measurements.

==> comments.tex <==
Reviewer(s)' Comments to Author:

Reviewer: 1

Comments to the Author
This paper discusses the FHD/Eppsilon software/pipeline methodology. It gives an excellent and detailed description of an important 21-cm processing pipeline, is generally easy to read and a useful reference. I do have a relatively large number of (mostly small) comments.

This is not the first and only 21-cm pipeline, so it would be helpful to have the goals and key features of this pipeline more prominently written down: what distinguishes this pipeline from other pipelines? I suggest to add this to the introduction and possibly as one line in the abstract. Key features to me seem the (enhanced) calibration methods to avoid spectral contamination from unmodelled sources, its use for in-depth verification, and its visibility-based but direction independent model subtraction. On the other hand, it seems the pipeline is not aimed at recovering the foreground-contaminated modes. If future plans for the pipeline exist, providing these (sect 8) would help in understanding the direction in which the pipeline is going.

%
Distinguishing characteristics have now been included in the intro and abstract. Potential future plans/avenues of the pipeline have been inserted into the text where they are most appropriate. There are no current plans to recover foreground-contaminated modes per se.
%

The tests are a bit simple. Since error propagation seems a defining feature of the pipeline, one of the things that I believe is missing from the tests, is to show a 1D power spectrum plot including error bars, e.g. as in Figure 7 (but in dimensionless units. Fig 6 does show the results of error propagation in a 2D plot, but is not easy to interpret). If possible, an upper limit on some set of data (can be small) that allows comparing with other results would also be helpful.

%
Figure 7 has been updated to include 2sigma errors and to be in mK squared. 

This now allows for qualitative comparison of upper limits, and they are comparable to Jacobs et al. 2016 for the same amount of data.

We will avoid making an explicit upper limit since this amount of data is for representative purposes only. We would prefer this paper to be about the analysis rather than the resulting limit; papers using FHD/eppsilon with a more competitive data set will be released in the future.  
%

The bandwidth gaps (which seem not to be simulated) result in strong excess power. From the results shown, it appears that this can be a major problem at least for analyzing MWA data. Is this software more affected by these gaps compared to other methods (for example because of not doing a full maximum likelihood inversion along the frequency axis)? In particular from Fig 7 it seems that deeper upper limits are inaccessible. This needs to be discussed in the paper.

%
Yes, this method is more affected. A paragraph has been added in Section 7 that states this and describes potential avenues for recovering affected modes in the future.

Figure 7 shows in the model that some modes will still be theoretically accessible even with coarse band structure. We have now pointed this out in Section 7.
%

The math is a bit confusing (details below), and the use of non-formal symbols such as "right arrow" should be avoided.

%
We have addressed the comments below and removed the majority of right arrows.
%

Comments from beginning to end:

page 1
Left side, 3rd line from bottom: "Fourier aliasing"
Reading the paper further I think I understand what is meant here, but at this point it is a term which can mean several things: please clarify.

%
We have changed the term to "spatial/frequency transform artifacts" to be more specific, since both spatial Fourier transforms and frequency Fourier transforms can introduce systematics.
%

page 2
Under bullet 3 of "B before antenna" : "Time correlations [caused by RFI]" this is somewhat of a confusing way of describing RFI; better say for example "unmodelled signals from RFI".

%
Done
%

Footnote 2 & text: Meaning of D ("errors in expected nominal configuration") is a bit unclear. According to Footnote 2, Hamaker uses it for including (modelled) polarization leakage, but this work absorbs that into C? Does that mean that D is defined as errors in the beam model? If not, where are those included?

%
Hamaker does not model any polarization leakage, and thus all polarization leakage from their point-of-view is an error. We have modified the footnotes to be more clear, and have condensed it into one footnote. We have also made it more clear that D is defined as errors to the expected configuration *and* beam model.
%

Page 3
3.1 In https://arxiv.org/abs/1901.04752 it is argued that flagging can cause bias. Is this relevant for the Eppsilon/FHD methodology as well ?

%
Since FHD/eppsilon does not use inverse-variance weighting of the visibilities, the contamination is lower than the expected EoR level as shown in Offringa et al 2019. This is a very important result, so we have added a paragraph for clarity.
%

line 14 under 3.2, and equation 2:
".. PP' = {P1 P2 , P1 P2' , P1 P2, P1' P2'} .."
This definition is a bit confusing. Is this supposed to define the product of P and P', or is PP' a name? Is the subscript supposed to define an antenna index? Should it be a vector (bold)? Is this supposed to mean that the authors are decomposing the two dimensional sky into the product of one dimensional functions? I think this part needs a bit of rewriting to be consistent with the math and to clarify.

%
We agree that the designation PP' is confusing. PP' more accurately defines a set, rather than a product. The real product comes from the visibility correlation between two elements A and B. We've modified the coherency/correlation domain polarisation to be called P wherever it occurs in the document, and we've also added it as a set in Table 2.

The subscript is supposed to be an antenna index, so we've changed it to be A and B to be consistent with the rest of the document.

P is the set of possible element polarisations that contribute to the visibility. We've changed the wording/equation to highlight that we assume two physical components (typically dipoles) named p and q (for generality). A visibility can be generated from dipole p from element A and dipole p from element B, dipole p from element A and dipole q from element B, etc. This explicitness also means that the only vectors in the equation are the Jones matrices. We believe this formulation is now much clearer.
%

I think Eq. 2 can be written easier and clarified. The generalization of this formula into Ps is probably more confusing than helpful: JP1->i seems not to be the same as JP1->j when i=j (if I interpret the formula correctly). The inclusion of f as parameter in C is not consistent: technically, the Js are also a function of f, so it should either be included everywhere or left out. It should be clarified what the square root operation of a matrix is: an element-wise matrix operation? Two lines below Eq. 2: "...as a function of the coordinate system" do the authors really mean a function of the coordinate "system", or should it be reworded?

%
Eq 2 has been modified to be clearer. We've changed the use of Ps (see previous response). We've also removed (x,y,f) and stated explicitly in the text that the matrices are a function of (x,y,f). Also, we state explicitly that all operations are element-wise operations, which was not clear before. We remove the use of "coordinate system:" it was confusing and it naturally fell out during the rewrite.
%

Page 4
Line 11: "This is achievable by hyperresolving, down to typically 1/7000 λ. "
Please also specify the (typical) cellsize or the hyperresolving factor, because the 1/7000 lambda value is on its own not very informative.

%
The typical gridding resolution has been added to the sentence. 
%

Last sentence of 3.2: "As long as the proper normalizations are taken into account in power weighting estimation, of the instrumental a modified gridding response. "
It also convolves/correlates the k-perpendicular axis.

%
A sentence has been added to alert the reader that this will cause pixel correlations, and to point to the section where this is explored in the power spectrum.
%

Start of 3.3: ", FHD simulates all reliable sources out to typically 1% beam level in the primary lobe and the sidelobes"
Can the (typical) simulated fov be included at this point? (The use of plural "sidelobes" seems to suggest that the full sky is simulated, but I'm not sure this is what the authors mean.)

%
A typical fov for 1% beam level of the MWA Phase I has been added for context. The plural use of sidelobes indicates that as much of the sky is simulated to simulate out to 1% beam level, which could include multiple sidelobes. We think the example makes the text clearer as to the intent.
%

Right side, line 3: Faraday rotation can also affect unpolarized sources when the Faraday rotation is different between different antennas. An additional assumption that the authors make is therefore that this is insignificant.

%
We now state this assumption in the text. We also switch the ordering of the "unresolved sources" paragraph and the "source position offsets" paragraph to introduce complications due to the ionosphere next to the stated assumption. We think that it's now more clear that removing observations with structured ionosphere helps to mitigate both O and F. 
%

Right side, line 15: "We disregard source position offsets O, a contamination resulting from ionospheric distortions. This assumption is only valid..."
Please reword this. The effect of O is decreased or minimized.

%
We have reworded it to say that the effect is minimized.
%

Right side, halfway: "..and this process is repeated for each observation to account for w-terms"
Better would be to say w-terms are "minimized". I assume there is some non-coplanarity in the MWA, and the observation is also of finite duration.

%
We agree that there is ambiguity. We have modified the term "w-terms" to be "w-terms associated with the instantaneous measurement plane" to indicate the specific type of w-terms we are mitigating. "Instantaneous measurement plane" describes the plane of the observation pointing, and thus does not included individual element altitude variation from the plane. That being said, we prefer there to be no misinterpretation, so we have also added "minimize" as suggested.
%

Page 5
Above eq 5, where A and B are defined. The definition of A and B is incorrect, as they are used as iterants in Eq 5, not sets themselves. This should be rewritten/reworded, for example something of the form "given the set of antennas A={...}, a and b iterate over all elements of A," etc, and correct Eq 5 accordingly. The same holds for PP' (this relates to an earlier comment about PP'). This also applies to table 2.

%
We have rewritten this notation. a and b now iterate through all elements of sets A and B, and a and b are used in Eq 5. Similarly, p and q now iterate through all elements of the set P. This has been changed in all instances where it occurs. 
%

Second line of 3.4.1: "Equation 7 can be used to solve for the instrumental gains for all frequencies and polarisations independently."
An earlier assumption was that the sky is unpolarized, so I assume this makes it impossible to calibrate all polarisations. It appears the authors (only) process XX and YY independently. Please add.

%
We explain under Equation 8 that we only solve for linear polarisations typically. We have added a phrase to "Optionally, a full polarisation treatment can be used" to indicate that polarised sources would be required. At the beginning of Section 3.4.1, we talk about polarisations of Eq 7 in general, and to not lose generality (or the various options that can be performed, though atypical), we have kept that intact. 
%

Page 7
Under eq 8: PP' -> PP
From context I gather this means something similar to "we assume no off-diagonally polarized power", but it should be clarified.

%
That is correct. We have clarified with an example.
%

Right side, 11 lines under Eq 10: "Van Vleck corrections"
What do the authors mean with this? A citation would be useful.

%
A citation has been added. We've added the adjective "quantisation" to indicate the nature of Van Vleck errors. Van Vleck corrections are corrections made to the correlator quantisation losses using the assumption that measurements are drawn from a Gaussian distribution.
%

Page 8
Eq 13: The right side term is divided by a scalar before taking the arg, which seems unnecessary.

%
We agree. It has been removed.
%

Above eq 14: "hyperfine DFT"
The term DFT is used in different ways: it can mean both discrete or direct FT, please fix this throughout the paper.
There's a mention that this is done for each observation. Why is this?

%
We agree. DFT has been defined throughout the paper. We are referring to the discrete Fourier transform in this instance.

In general, this fit is performed per observation because the reflection amplitude has a phase which can change depending on the stability of the instrument. For example. this cable reflection fitting was developed using a specific set of MWA data where various hardware was updated throughout the season, and thus sometimes cable reflection phases would change. This is more detail than we want to go into in this work, so we have removed the "for each observation" phrase for generality. In the following paragraph, we have added a sentence that we can optionally average the cable reflections to get better numbers in order to be more consistent with the layout of the bandpass section. 
%

Page 9
Above eq 15: "Whether or not ... fine-frequency bandpass"
The reason to solve for fine-frequency bandpass on top of the other solved effects is bit unclear to me. This is to solve the fine structure of Fig 2? What instrumental effect is solved by this fit, the filter band edges?

%
The reasons for solving for a fine-frequency bandpass are discussed in 3.4.2. The term "fine-frequency" is jargon and has been removed so that it is more obvious that we are talking about the bandpass introduced in 3.4.2. We have also added more information in 3.4.2 about the bandpass accuracy requirements, which motivates the reason for solving for calibration parameters carefully. 

The instrumental effects that are captured by the bandpass fit are many and varied, and we surely don't know all the effects. It is also highly instrument-specific. We have not added any more description of the potential instrument parameters that the bandpass captures to keep generality and to be within the scope we are trying to create.
%

5 lines above 3.4.6: "...for bit noise"
At what stage is the bit noise occurring? (After the ADC? During/after the correlator?)

%
This can be any bit truncation noise, and it will depend on the instrument. We have added a phrase to indicate that the bit noise can occur anywhere there is bit truncation. 
%

3.5, line 5: "We convolve visibility values by the beam sensitivity..."
The beam is calculated as full matrix, but the polarizations are independently processed. It is therefore unclear if this is a scalar correction, or are the beam responses as full matrices corrected?

%
The beam is calculated in the coherency domain as discussed in Section 3.2 (XX,XY,YX,YY for the MWA). Therefore, each polarisation can be processed individually, which would not be the case if we generated the beam in Stokes. We have modified the sentence to include this designation explicitly to avoid confusion.
%

Right after: "In essence, this takes integrated values and de-integrates them given our knowledge of the beam in uv-space."
This seems to suggest the beam is corrected for (convolved with the inverse of the beam sensitivity), whereas the previous sentence mentions that it is the other way around. If I interpret correctly that the authors indeed apply the inverted beam during gridding of the visibilities, this needs some explanation. Doing so implies that areas within the fov that have low sensitivity are upweighted. Binning visibilities his way is not optimal weighting. 

%
This was not our intent, so we have modified the sentence accordingly. We are trying to create estimates of the original spatial uv-response of the visibility before it was integrated by the element during measurement, and approximating this to a set of uv-grid points. The modified sentence is now more clear (and avoids the use of the term "de-integrates," which is not proper).
%

Page 10
9 lines above 3.6: "we interpolate to HEALPix pixel centers"
What method is used for interpolation?

%
We use bilinear interpolation. This has been added to the text.
%

Page 12
Line 7: "..altitude variations must be captured with accurate calibration phases."
Does this also imply that the visibilities are calibrated to have no altitude differences?
The phase corrections due to altitude variations vary over the field of view (even in a snapshot), so an additional requirement is that the FOV is small.

%
"Captured with accurate calibration phases" was not correct. We have modified this, and given more information. FHD/eppsilon assumes coplaner instruments, but does not require the FoV to be small. Instead, we require the instrument to be very coplaner or to use the unique kernel generation mentioned in Section 3.2. We have provided an estimate for how coplaner the MWA Phase I instrument is, and have indicated that it is not *currently* a dominating systematic to the analysis. This subtly indicates that this might need to be accounted for in the future. 
%

line 12: "..in εppsilon and CHIPS are unique in this respect."
I doubt that these pipelines are the only ones doing this (for example https://iopscience.iop.org/article/10.3847/1538-4357/aa63e7/meta and https://academic.oup.com/mnras/article/478/3/3640/4995230 seem both to do something similar).

%
The Patil et al 2017 paper bootstraps their errors from the Stokes V image. 

The Mertens et al 2017 paper could be able to show simulated noise generated from data visibilities alongside data analyses (which would essentially be the same as analytical propagation). Mertens et al seem to indicate that bootstraping from Stokes V would still be used for non-simulation scenarios. 

However, we agree that this designation is too bold. It also would probably not be true in the future. We've modified the sentence to say that it is "uncommon."
%

8 lines under 5.1: "We then Fourier transform the integrated image back into uv-space.."

Is this from HEALPix? Or from another reprojection? Is a window applied during the FT?

%
It is from HEALPix cube. We have added this detail in the text. 

The Tapered Gridded Estimator described in Section 3.2 acts as a window in image space. We must apply this window to the beam in order to get our variance cubes used for error propagation correct. This is now described in the text.
%

In the next sentence, do the authors mean "direct" instead of "discrete Fourier transform"?

%
We do. The text has been updated.
%

Page 13
Line 5: "We can confirm this simplification by comparing the analytic noise propagation to the observed noise in the power spectrum (§6.1). Their ratio very close to 1, indicating that our assumption is valid."
This could be a useful test, but it is not a proof of independence and this paragraph should be reworded or removed.
The ratio seems to vary at least between 0.5 and 2. This could be partially just due to errors on the errors, thereby decreasing the usefulness of this test, but stating that it is very close to one is misleading.

%
We agree. We've updated the text to indicate that it investigates the strength of the correlation rather than completely disproves its existence. 

In Section 6.1 (where the 2D noise ratio is described) we now go into more quantitative detail on the ratio in the most important modes. The ratio is approximately 0.9, indicating that we slightly overestimate our noise due to our no-correlation assumption. The range of the 2D ratio plot has now been updated to be between 0.5 and 2 to be more useful.
%

5.3, line 13: "To preserve the DC term in the power spectrum, we add this value after our spectral transform."
The mean is not independent of the other parameters in a non-uniformly sampled transform. It also appears the mean is not actually used/displayed. Is this nevertheless useful?

%
We remove the mean to reduce leakage on the spectral transform, not for display purposes. We add more detail on why we do this in the text. 

We agree that the mean could potentially be not-independent. We've added a discussion on signal loss, what that means for this particular mode, and finally pointed to the signal loss section as proof that removing the mean before the spectral transform and adding it back in to the DC mode does not result in signal loss. 
%

Above eq 24: "we add each squared eigenfunction together"
Is 'eigenfunction' supposed to refer to the values of the periodogram?
Same sentence: "weighting by the variance of their respective Rayleigh distributions."
An amplitude is Rayleigh distributed, but this is in power, which would follow an exponential distribution. Please reword this and the previous sentence to clarify what is meant.

%
We feel like this description of the Lomb-Scargle was confusing and not necessary. We've removed most of this discussion from the text. 
%

Under 5.4: "We now have the maximum likelihood estimate for the.."
The power spectrum estimates as described are not the maximum likelihood estimates (for example: the Lomb-Scargle method produces the ML estimate when there is only one mode in the data, but this does not hold for a 21-cm power spectrum)

%
We agree. We've changed this to emphasis that they are power spectra estimates, not maximum likelihood estimates.
%

Page 14
Above Fig 4: "delay in nanosecond"
Fig 4 does not have values on the delay axis.

%
We have now fixed this.
%

Page 16
Fig 6. Using 2 orders of magnitude for the ratio in the bottom right is not very useful. Better to use a scale of 0.5 to 2.

%
We agree. We have modified the figure.
%

Page 17
Under 7, near bullet points. How are the EoR signals simulated? Is it from a simulations or is it just a statistical realisation of a Gaussian field? How is the "EoR signal" transferred to visibility space? If it is degridded, there could still be bias in the normalization, or in the gridding and degridding operation, that cancels out (which has probably been verified in other ways, and good to mention this).

%
The EoR signal is simulated from a Gaussian field, and this has been added to the text for clarity. The EoR signal is transferred to visibility space via degridding. We agree that the signal loss simulation therefore does not test the validity of the beginning simulation, and this has been added to the text. We explicitly state that the encoded instrumental effects are not validated, along with the sky temperature taken from the model sky.
%

Page 18
Fig 7: The left 2D PS has negative values whereas the right plot does not. If the left one has been corrected for noise-bias please mention this.
The left image should have a colorbar.
The quantity along the y-axis of the right image should be Delta (squared) instead of P. Error bars should be added.

%
The left 2D PS *has not* been corrected for a noise bias. The right plot does have negative values, they appear at high k. We could have more noise-dominated bins at low k in the 1D plot if we excluded the horizon, but we feel as though that's outside of the scope of what we want to achieve with this figure. We don't want to make limits on the EoR with this data, we only want to prove the usefulness of FHD/eppsilon. 

We've added error bars, which help to show that there are more noise-dominated regions than that could be deciphered from the original plot previously. We've also changed the 1D units to be Delta squared, and have added a color bar to the 2D plot.
%

Page 19
Fig 9: Please mention there are no bandwidth gaps in this simulation (if that is correctly assumed).
This plot should also have units of mK (squared) along the y-axis.
I'm not sure a factor of two would be visible in this plot (that covers 9 orders). It would therefore be useful to show a difference plot instead.
There appears to be extra power at high k for the foregrounds+EoR case. Where is this coming from?

%
We've now mentioned that there are no channeliser effects, and that future studies can take into account channeliser effects.

Plot units have been changed to mK squared.

We think that future simulations will be required to understand a wider range of effects, and our current simulation of point sources and EoR is extremely simple. Therefore, we would like to wait for future papers before making a 2D difference plot of the simulations. Currently, the simulations fluctuate within 1 mK squared for a some modes when compared to the "EoR in pipeline" test (which is easy to compare to, since it's on the same binning scheme as the other tests).

The extra power at high k comes from a gridding resolution systematic found by Beardsley et. al. 2016. This has been added to the text.
%

==> extra_comments.tex <==
Reviewer(s)' Comments to Author:

Reviewer: 1

Comments to the Author
I have one more comment, related to this answer by the authors:

%
Yes, this method is more affected. A paragraph has been added in Section 7 that states this and describes potential avenues for recovering affected modes in the future.

Figure 7 shows in the model that some modes will still be theoretically accessible even with coarse band structure. We have now pointed this out in Section 7.
%

Two small things about the new paragraph:
"This is a consequence of the lack of inverse-variance weighting."
- I would explicitly add wording similar to "during the line-of-sight transform", because inverse-variance weighting can be done at various stages.

Directly after:
"While this allows εppsilon to avoid potential ambiguity associated with inverse-weighting, ..."
- inverse-weighting should be "inverse-variance weighting"
- I'm not sure what "potential ambiguity" refers to, a degenerate inversion? Please clarify, or alternatively remove the sentence (it doesn't seem to add information).
